From Monopoly to Competition: Optimal Contests Prevail

We study competition among contests in a general model that allows for an arbitrary and heterogeneous space of contest design, where the goal of the contest designers is to maximize the contestants' sum of efforts. Our main result shows that optimal contests in the monopolistic setting (i.e., those that maximize the sum of efforts in a model with a single contest) form an equilibrium in the model with competition among contests. Under a very natural assumption these contests are in fact dominant, and the equilibria that they form are unique. Moreover, equilibria with the optimal contests are Pareto-optimal even in cases where other equilibria emerge. In many natural cases, they also maximize the social welfare.

==> 2020 fall_ Contests design/notation.tex <==
%% General machinery
\newcommand{\AutoAdjust}[3]{{ \mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }}
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}% {\left[{#1}\right]}
\newcommand{\Ex}[2][]{\operatorname{\mathbbm E}_{#1}\InBrackets{#2}}
\newcommand{\Prx}[2][]{\operatorname{\mathbf{Pr}}_{#1}\InBrackets{#2}}
\def\prob{\Prx}
\def\expect{\Ex}
\newcommand{\probq}[2]{x_{#1}\AutoAdjust{(}{#2}{)}}
\newcommand{\cumprobq}[2]{X_{#1}\AutoAdjust{(}{#2}{)}}
\newcommand{\super}[1]{^{(#1)}}
\newcommand{\dd}{\mathrm{d}}  % for integrals
\newcommand{\given}{\;\mid\;}
\newcommand{\eps}{\varepsilon}
\renewcommand{\vec}{\bm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareRobustCommand\iff{\;\Longleftrightarrow\;}

\newcommand{\noaccents}[1]{#1}
\newcommand{\newagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}



\newcommand{\newvecagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{\boldsymbol{#3}}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

% need \usepackage{mathtools}
\DeclarePairedDelimiter\paren{(}{)}
\DeclarePairedDelimiter\bkt{[}{]}
\DeclarePairedDelimiter\set{\{}{\}}
\DeclarePairedDelimiter\ang{\langle}{\rangle}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}	
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
% usage:
%   \paren{abc} = (abc), where the size of "(", ")" is default. 
%   \paren*{abc} = (abc), where the size of "(", ")" is adjusted automatically. 
%   \paren[\big]{abc} = (abc), where the size of "(", ")" is \big. 
%   \norm{a} = ||a||, where the the size of "||" is default.  Use \norm*{a} to adjust the size automatically. 


\newagentvar{val}{v}
\newagentvar{bid}{b}
\newagentvar{dist}{F}
\newagentvar{alloc}{x}
\newagentvar{util}{u}
\newagentvar{pay}{p}
% You can define a vector u by \newagentvar{name}{u}
\newagentvar{ability}{a}
\newagentvar{effort}{e}

\DeclareMathOperator{\Rev}{Rev}
\DeclareMathOperator{\SW}{SW}
\DeclareMathOperator{\OPT}{OPT}

\newcommand{\redcom}[1]{\textcolor{red}{[#1]}}
\newcommand{\bluecom}[1]{\textcolor{blue}{[#1]}}

\DeclareMathOperator{\naturals}{\mathbb{N}}

\DeclareMathOperator{\posreals}{{\mathbb{R}_{+}}}

\DeclareMathOperator{\reals}{{\mathbb R}}


\newcommand{\reward}{R}
\newcommand{\cf}{\rho}
\newcommand{\family}{{\mathcal F}}

\newcommand{\bin}{\mathrm{Bin}}
\newcommand{\cutil}{\gamma}
\newcommand{\mrd}{\mathrm{MRD}}
\newcommand{\MRD}{\mathrm{MRD}}
\newcommand{\wta}{\mathrm{APA}}
\newcommand{\WTA}{\mathrm{APA}}
\newcommand{\AVERSE}{\mathrm{averse}}

\newcommand{\Supp}{\mathrm{Supp}}

\newcommand{\yotam}[1]{{\color{red}{Yotam: #1}}}
\newcommand{\ron}[1]{{\color{blue}{Ron: #1}}}
\newcommand{\deng}[1]{{\color{green}{Xiaootie: #1}}}
\newcommand{\hongyi}[1]{{\color{cyan}{Hongyi: #1}}}

